Perfect Numbers in ACL2

A perfect number is a positive integer n such that n equals the sum of all positive integer divisors of n that are less than n. That is, although n is a divisor of n, n is excluded from this sum. Thus 6 = 1 + 2 + 3 is perfect, but 12 < 1 + 2 + 3 + 4 + 6 is not perfect. An ACL2 theory of perfect numbers is developed and used to prove, in ACL2(r), this bit of mathematical folklore: Even if there are infinitely many perfect numbers the series of the reciprocals of all perfect numbers converges.

==> eptcsdata.tex <==
\providecommand{\firstpage}{53}
\providecommand{\publicationstatus}{M. Kaufmann and D. Rager (Eds.): ACL2 Workshop 2015 (ACL2 2015).\\
EPTCS 192, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.192.5}{10.4204/EPTCS.192.5}}
\pdfoutput=1

